Uncertain Machine Ethics Planning

Machine Ethics decisions should consider the implications of uncertainty over decisions. Decisions should be made over sequences of actions to reach preferable outcomes long term. The evaluation of outcomes, however, may invoke one or more moral theories, which might have conflicting judgements. Each theory will require differing representations of the ethical situation. For example, Utilitarianism measures numerical values, Deontology analyses duties, and Virtue Ethics emphasises moral character. While balancing potentially conflicting moral considerations, decisions may need to be made, for example, to achieve morally neutral goals with minimal costs. In this paper, we formalise the problem as a Multi-Moral Markov Decision Process and a Multi-Moral Stochastic Shortest Path Problem. We develop a heuristic algorithm based on Multi-Objective AO*, utilising Sven-Ove Hansson's Hypothetical Retrospection procedure for ethical reasoning under uncertainty. Our approach is validated by a case study from Machine Ethics literature: the problem of whether to steal insulin for someone who needs it.

==> Algorithms/oldMOLAO.tex <==
\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}
\begin{minipage}[t]{\textwidth}
  \raggedright
  \textbf{Input}: Multi-Moral SSP $\langle S, A, P, s_0, H, M, C, L, R, \budget, \goals \rangle$, heuristic $h$\\
  \textbf{Output}: Optimal moral policy, \policy
\end{minipage}


\begin{algorithmic}[1]
\State$\vec{W} \gets \{ \{ h_c(s) : \forall{c\in C}\} \}$; $F \gets \{(s_0,0)\}$; $I \gets \emptyset;$
\State $\mathfrak{A}[t](s) \gets \emptyset : \forall_{s\in S, t \in \{0,...,H-1\}}; \mathfrak{A}[0](s_0) \gets A$
\Do
    \State $\vec{W}' \gets \vec{W}$; $Z \gets \text{postOrderDFS}(I\cup F, \mathfrak{A})$
    \For{$s, t \in Z$}
        \State$\vec{W}[t](s) \gets \{ \vgatherf^{\boldsymbol{W}[t+1]}(s,a) :\forall{a \in A, \boldsymbol{W} \text{ from } \vec{W}} \}$
        \State $\vec{W}[t](s) \gets \{\vec{W} \in \vec{W}[t](s) : \vec{W}_R[t](s) < \budget \}$
        \State $\vec{W}[t](s) \gets \text{pprune}(\vec{W}[t](s))$
        \State $\mathfrak{A}[t](s) \gets \{a \in A : \vgatherf^{\boldsymbol{W}[t+1]}(s,a) \cap \vec{\boldsymbol{W}} \neq \emptyset \}$
        \State $F \gets (F \backslash \{(s,t)\}) \cup \{s' \in S \backslash I : \exists_{a\in A}P(s,a,s')>0\}$
        \State $I \gets I \cup \{(s,t)\}$
    \EndFor
\doWhile{$((F \cap Z) \backslash G = \emptyset) \land (\vec{W} \approx \vec{W'})$}
\State $\Pi \gets$ Extract policies $\pi$ from $\vec{\boldsymbol{W}}$
\State $\phi^\pi \gets$ Extract Histories from $\pi$, $\forall{\pi \in \Pi}$
\State \Return $\policy \gets \text{MEHR}(\Pi, \{\phi^\policy : \forall{\policy \in \Pi\}} \})$
\end{algorithmic}


==> Figures/worked_MEHR.tex <==
\usetikzlibrary{positioning, arrows.meta, calc}
\begin{tikzpicture}[
  grow=down,
  level 1/.style={sibling distance=4cm, level distance=1cm},
  level 2/.style={sibling distance=2cm, level distance=1.5cm},
  level 3/.style={sibling distance=2cm, level distance=2cm},
  edge from parent/.style={draw,-latex},
  root/.style={circle,draw, minimum size=1cm, align=center},
  outcome/.style={circle,draw, minimum size=1cm, align=center, text width=1cm, font=\footnotesize}, % Set minimum size for circle nodes
  parallelogram/.style={draw, trapezium, trapezium angle=70, minimum height=1cm,  trapezium stretches=true, trapezium stretches body=true, align=center, text width=1cm, font=\footnotesize}, % Set minimum height and width for parallelogram nodes
  attack/.style={line width = 1pt, -{Latex[width=3mm]}},
  argument/.style={draw, rectangle, align=center},
  utilNonAcc/.style={color=red, align=center},
  deonNonAcc/.style={color=blue, align=center}
]




\newcommand{\widthFactor}{1.5}
\newcommand{\heightFactor}{0.8}

\node[argument] (pi2_h3) {$Arg(\policy_2, h_3)$} ;
\node[argument, right=\widthFactor * 1cm of pi2_h3] (pi2_h4) {$Arg(\policy_2, h_4)$};
\node[argument, right=\widthFactor * 1cm of pi2_h4] (pi2_h5) {$Arg(\policy_2, h_5)$};
\node[argument, right=\widthFactor * 1cm of pi2_h5] (pi2_h6) {$Arg(\policy_2, h_6)$};


\node[argument, above=\heightFactor * 1cm of pi2_h4] (pi1_h1) {$Arg(\policy_1, h_1)$};
\node[argument, right=\widthFactor * 1cm of pi1_h1] (pi1_h2) {$Arg(\policy_1, h_2)$};


\draw[->, line width=0.1mm, color=blue, dashed, -{Stealth[width=2mm]}] (pi1_h2.south) to[looseness=1] (pi2_h3.north);

\draw[->, line width=0.1mm, color=blue, dashed, -{Stealth[width=2mm]}] (pi1_h2.south) -- (pi2_h4.north);
\draw[->, line width=0.1mm, color=blue, dashed, -{Stealth[width=2mm]}] (pi1_h2.south) -- (pi2_h5.north);
\draw[->, line width=0.1mm, color=blue, dashed, -{Stealth[width=2mm]}] (pi1_h2.south) -- (pi2_h6.north);

\draw[->, line width=0.1mm, color=red, -{Stealth[width=3mm]}] (pi2_h4.north) -- (pi1_h1.south);

\node[utilNonAcc, above=\heightFactor * 0.2cm of pi1_h1] (n) {\small$+P(h_1)=0.4$};

\node[deonNonAcc, below=\heightFactor * 0.1cm of pi2_h3] (m) {\small$+P(h_3)=0.6$};
\node[deonNonAcc, below=\heightFactor * 0.1cm of pi2_h4] {\small $+P(h_4)=0.15$};
\node[deonNonAcc, below=\heightFactor * 0.1cm of pi2_h5] {\small$+P(h_5)=0.15$};
\node[deonNonAcc, below=\heightFactor * 0.1cm of pi2_h6] {\small$+P(h_6)=0.05$};

\path (pi1_h1) -- (pi1_h2) coordinate[midway] (midpoint_pi1);
\path (pi2_h4) -- (pi2_h5) coordinate[midway] (midpoint_pi2);

\node[color=blue, below=\heightFactor * 1.4cm of midpoint_pi2] {$=1.0$ non-acceptability on $\pi_2$.};
\node[color=red, above=\heightFactor * 1.4cm of midpoint_pi1] {$=0.4$ non-acceptability on $\pi_1$.};

%\node[color=red] at (0,1) {$=0.4$ non-acceptability on $\pi_2$.};

\end{tikzpicture}

